Great Power, Great Responsibility: Recommendations for Reducing Energy for Training Language Models

The energy requirements of current natural language processing models continue to grow at a rapid, unsustainable pace. Recent works highlighting this problem conclude there is an urgent need for methods that reduce the energy needs of NLP and machine learning more broadly. In this article, we investigate techniques that can be used to reduce the energy consumption of common NLP applications. In particular, we focus on techniques to measure energy usage and different hardware and datacenter-oriented settings that can be tuned to reduce energy consumption for training and inference for language models. We characterize the impact of these settings on metrics such as computational performance and energy consumption through experiments conducted on a high performance computing system as well as popular cloud computing platforms. These techniques can lead to significant reduction in energy consumption when training language models or their use for inference. For example, power-capping, which limits the maximum power a GPU can consume, can enable a 15\% decrease in energy usage with marginal increase in overall computation time when training a transformer-based language model.

==> batch_table.tex <==
\begin{table*}[h]
\vspace{-0.1in}\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Batch Size & \multicolumn{2}{c|}{8} & \multicolumn{2}{c|}{16} \\
\hline
Max Power & Time (s) & Energy (kWh) & Time (s) & Energy (kWh) \\
\hline
100W & 16402 & 5.91 & 16517 & 6.08 \\
150W & 12917 & 5.82 & 12468 & 5.74 \\
200W & 12290 & 6.48 & 9073 & 5.89 \\
250W & 12022 & 6.82 & 8736 & 6.36 \\
% 100W & 16401.89 & 5.909091 & 14841.96 & 5.944495 \\
% 150W & 12917.38 & 5.8163035 & 17438.44 & 6.78102737 \\
% 200W & 12290.08 & 6.476801 & 9164.39 & 5.914852 \\
% 250W & 12021.92 & 6.8178108 & 8811.0 & 6.45224781 \\
% 100.0, 8, 10.0, 5.909091857120838, 16401.89,
% 150.0, 8, 10.0, 5.816303561259727, 12917.38,
% 200.0, 8, 10.0, 6.476801246670824, 12290.08,
% 250.0, 8, 10.0, 6.817810857755557, 12021.92,
% 100.0, 16, 10.0, 5.944495678651395, 14841.96,
% 150.0, 16, 10.0, 6.781027370119442, 17438.44,
% 200.0, 16, 10.0, 5.9148525112222226, 9164.39,
% 250.0, 16, 10.0, 6.452247819079171, 8811.0,
\hline
\end{tabular}
\caption{\label{tab:batch_table} Observed energy consumption and training time when training BERT with batch sizes of either 8 or 16 per-GPU. Batches of 32 and larger exceeded available memory.}
\end{table*}

==> experiments_list.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}
{Parameters} \\
\hline
Power Levels & 100W, 150W, 200W, 250W \\
\hline
\# GPUs & 64, 128, 256, \jpm{384}, 424 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> plots_inference.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.5\textwidth]{plots/plot_bars_inference.png}
    \caption{\label{fig:plotinf} Comparison of time to complete inference and energy consumption on a test set among different maximum power thresholds. Values are percentage relative to default (250W) settings.}
\end{figure}

==> plots_scratch.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=2.25in]{plots/plot_bars_best.png}
    \caption{\label{fig:barplotbest} \jpm{This is a placeholder for model selection plots.}}

\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.5in]{plots/plot_bars_inference_3.png}
%     \includegraphics[width=1.2in]{plots/plot_bars_inference_2.png}
%     \caption{\jpm{Put numbers on top of bars and be clear that this is TOTAL energy used}}
%     \label{fig:barplotinf}
% \end{figure}

==> table.tex <==
\begin{table*}[ht]
\caption{Add caption here}
\centering
\begin{tabular}{||p{0.2\linewidth} | p{0.3\linewidth} |  p{0.15\linewidth} |  p{0.1\linewidth} |  p{0.1\linewidth} ||} 
 \hline
 Intervention & Description & Performance Impact & Accuracy Impact & Energy Impact \\ [0.5ex] 
 \hline\hline
 Hardware capabilities & Use technique such as power capping or frequency limiting & -5\% & 0 & -15\% \\ 
 \hline
 Efficient Scheduling & Use changes in datacenter efficiency to improve efficiency  & 0\%* & 0\% & -10\% \\
 \hline
 Intelligent Hardware Selection & AA & BB & CC & DD  \\
 \hline
 Early Stopping & AA & BB & CC & DD \\
 \hline
 \hline
 \textbf{Total} & AA & BB & CC & DD \\
 \hline
\end{tabular}
\end{table*}

==> training_table.tex <==
\begin{table}[ht]
\caption{Time and Energy usage of varying number of Epochs when training the BERT model. Results indicate approximately linear time and energy usage.}
\centering
\begin{tabular}{p{0.2\linewidth} p{0.2\linewidth}  p{0.25\linewidth}} 
 \hline
Number of Epochs & Training Time (s) & Energy (kWh)  \\
 \hline
 1 & 1232 & 0.67 \\ 
 2 & 2417 & 1.37 \\ 
 3 & 3671 & 2.05 \\ 
 4 & 4891 & \textcolor{red}{2.02} \\ 
 \hline
\end{tabular}
\end{table}
